Cost Analysis of Redundancy Schemes for Distributed Storage Systems

Distributed storage infrastructures require the use of data redundancy to achieve high data reliability. Unfortunately, the use of redundancy introduces storage and communication overheads, which can either reduce the overall storage capacity of the system or increase its costs. To mitigate the storage and communication overhead, different redundancy schemes have been proposed. However, due to the great variety of underlaying storage infrastructures and the different application needs, optimizing these redundancy schemes for each storage infrastructure is cumbersome. The lack of rules to determine the optimal level of redundancy for each storage configuration leads developers in industry to often choose simpler redundancy schemes, which are usually not the optimal ones. In this paper we analyze the cost of different redundancy schemes and derive a set of rules to determine which redundancy scheme minimizes the storage and the communication costs for a given system configuration. Additionally, we use simulation to show that theoretically-optimal schemes may not be viable in a realistic setting where nodes can go off-line and repairs may be delayed. In these cases, we identify which are the trade-offs between the storage and communication overheads of the redundancy scheme and its data reliability.

==> simul/combining-bandwidth-a.tex <==
\subfloat[MSR ($i=0$; $d=k$) Reed-Solomon~Codes]{\label{f:combband:msrlow}\includegraphics{simul/combining-bandwidth-msrlow.eps}}
\subfloat[MSR ($i=0$; $d=n-1$)]{\label{f:combband:msrhigh}\includegraphics{simul/combining-bandwidth-msrhigh.eps}}
\subfloat[MBR ($i=k$; $d=k$)]{\label{f:combband:mbrlow}\includegraphics{simul/combining-bandwidth-mbrlow.eps}}
\subfloat[MBR ($i=k$; $d=n-1$)]{\label{f:combband:mbrhigh}\includegraphics{simul/combining-bandwidth-mbrhigh.eps}}


==> simul/combining-redundancy-a.tex <==
\subfloat[MSR ($i=0$; $d=k$)]{\label{f:combred:msrlow}\includegraphics{simul/combining-redundancy-msrlow.eps}}
\subfloat[MSR ($i=0$; $d=n-1$)]{\label{f:combred:msrhigh}\includegraphics{simul/combining-redundancy-msrhigh.eps}}
\subfloat[MBR ($i=k-1$; $d=k$)]{\label{f:combred:mbrlow}\includegraphics{simul/combining-redundancy-mbrlow.eps}}
\subfloat[MBR ($i=k-1$; $d=n-1$)]{\label{f:combred:mbrhigh}\includegraphics{simul/combining-redundancy-mbrhigh.eps}}


==> simul/regenerating-red.tex <==
\subfloat[Redundancy for MSR codes.]{\label{f:redund:msr}\includegraphics{simul/regenerating-red-msr.eps}}
\subfloat[Redundancy for MBR codes.]{\label{f:redund:mbr}\includegraphics{simul/regenerating-red-mbr.eps}}
\subfloat[Value of n.]{\label{f:redund:n}\includegraphics{simul/regenerating-red-n.eps}}

